Relaxed Conditional Image Transfer for Semi-supervised Domain Adaptation

Semi-supervised domain adaptation (SSDA), which aims to learn models in a partially labeled target domain with the assistance of the fully labeled source domain, attracts increasing attention in recent years. To explicitly leverage the labeled data in both domains, we naturally introduce a conditional GAN framework to transfer images without changing the semantics in SSDA. However, we identify a label-domination problem in such an approach. In fact, the generator tends to overlook the input source image and only memorizes prototypes of each class, which results in unsatisfactory adaptation performance. To this end, we propose a simple yet effective Relaxed conditional GAN (Relaxed cGAN) framework. Specifically, we feed the image without its label to our generator. In this way, the generator has to infer the semantic information of input data. We formally prove that its equilibrium is desirable and empirically validate its practical convergence and effectiveness in image transfer. Additionally, we propose several techniques to make use of unlabeled data in the target domain, enhancing the model in SSDA settings. We validate our method on the well-adopted datasets: Digits, DomainNet, and Office-Home. We achieve state-of-the-art performance on DomainNet, Office-Home and most digit benchmarks in low-resource and high-resource settings.

==> background.tex <==
\section{Background}

\subsection{Generative Adversarial Net}

Generative Adversarial Net (GAN)~\cite{goodfellow2014generative} is one of the most popular generative models for unsupervised learning and achieves remarkable progress in image generation~\cite{arjovsky2017wasserstein,miyato2018spectral,brock2018large}. GAN employs a generator network $G$ that maps a latent vector $z$ to a real image $x$. A discriminator network $D$ is introduced to discriminate whether a sample is a real image or a  fake one and the generator tries to fool $D$. Formally, the GAN's objective function is
\begin{equation}
\label{eq:gan-objective}
\min_G \max_D V(D, G) = \mathbb{E}_{x \sim p(x)}[\log D(x)] + \mathbb{E}_{z \sim p_z(z)}[\log (1 - D(G(z)))],
\end{equation}
where $p(x)$ is a uniform distribution on the training data and 
$p_z(z)$ is a simple prior distribution.

\subsection{Triple Generative Adversarial Net}
\label{sec:triplegan-section}
 
In semi-supervised learning (SSL), we have a small set of labeled data $\mathcal{D}=\left\{\left(x_{i}, {y_{i}}\right)\right\}_{i=1}^{m_l}$, as well as a large set of unlabeled data $\mathcal{D}_{u} = \left\{\left(x_{i}^{u} \right)\right\}_{i=1}^{m_{u}}$. To leverage the unlabeled data, Triple-GAN~\cite{chongxuan2017triple} defines an adversarial game among three networks: a generator $G$, a discriminator $D$ and a classifier $C$. The generator and the classifier generate fake data given true labels and fake labels given true data, respectively. The discriminator tries to determine whether a label-data pair is from the true data distribution or not. The objective function of Triple-GAN is provided by
\setlength{\arraycolsep}{0.0em}
\begin{eqnarray}\label{eq:triple_gan_full}
\min_{C, G} \max_D U(C,G,D) = &\mathbb{E}&_{(x,y) \sim p(x, y)} [\log D(x, y)]
+ \alpha \mathbb{E}_{x \sim p_u(x)} [\log (1 - D(x, C(x)))] \nonumber \\
&+& (1-\alpha) \mathbb{E}_{y\sim p(y), z\sim p_z(z)} [\log (1 - D(G(y, z), y))] + R_{C},
\end{eqnarray}
where $p(x,y)$, $p_u(x)$ and $p(y)$ are uniform distributions over $\mathcal{D}$, $\mathcal{D}_{u}$ and all possible labels, respectively, $\alpha$ is a constant controlling the importance of generation and classification, and $R_C$ is the regular cross-entropy loss for the classification on labeled data. Theoretically, Triple-GAN proves that the fake label-data distribution produced by both $G$ and $C$ converge to the true data distribution $p(x,y)$. 
Readers may refer to the original paper~\cite{chongxuan2017triple} for more details.

==> conclusion.tex <==
\section{Conclusion}

In this work, we focus on two challenges in SSDA, including the label-inconsistency problem and the label-domination problem.
These two problems usually result in poor source image transfer and finally hurt the performance of the classification.
We  elaborately design Relaxed cGAN, which consists of a conditional discriminator, an unconditional generator, as well as a jointly trained classifier, to alleviate the two problems and eventually achieve satisfactory classification accuracy.
Empirically, Relaxed cGAN is able to generate diverse data in the target domain through adaptation, which leads to substantial improvements in classification.
Extensive experimental results show that the proposed Relaxed cGAN achieves state-of-the-art results on several widely adopted digit adaptation benchmarks, and shows competitive results on DomainNet under both low-resource and high-resource SSDA settings.
